Local Subspace-Based Outlier Detection using Global Neighbourhoods

Outlier detection in high-dimensional data is a challenging yet important task, as it has applications in, e.g., fraud detection and quality control. State-of-the-art density-based algorithms perform well because they 1) take the local neighbourhoods of data points into account and 2) consider feature subspaces. In highly complex and high-dimensional data, however, existing methods are likely to overlook important outliers because they do not explicitly take into account that the data is often a mixture distribution of multiple components. We therefore introduce GLOSS, an algorithm that performs local subspace outlier detection using global neighbourhoods. Experiments on synthetic data demonstrate that GLOSS more accurately detects local outliers in mixed data than its competitors. Moreover, experiments on real-world data show that our approach identifies relevant outliers overlooked by existing methods, confirming that one should keep an eye on the global perspective even when doing local outlier detection.

==> chapters/problem.tex <==
Detecting outliers in mixed datasets where several clusters are present can be very challenging when local outliers are hiding in or near different local clusters. Outliers can be overlooked when focusing too much on the local scope and outliers can also be overlooked when only considering the global scope of the data. 
A datapoint $x \in X$ can be an outlier in feature $f$ considering the neighbors of $x$, but not considering the whole dataset $X$. For example, a weather dataset with $365$ records where each record is a time-series of temperatures for one day for a specific year. The task for this dataset would then be to find time periods where the weather is considered outlying, which could be a very high temperature day in the winter but also an hour of a summer day with a very low temperature. In this weather dataset the overall measurements may vary a lot and due to this global variation local outliers may be overlooked when only considering the complete global space of days. However, if we only look at local feature subspaces (for example each hour of each day), a very low temperature hour in summer is likely very close to normal hours in autumn or spring, but should be considered an outlier if the rest of the summer and this day was beautiful weather with high temperatures.

Normally we are used to call a record $x$ an outlier when the probability of $x$ is low given the rest of the dataset, in this particular case we would also need to define a certain feature space.

\begin{definition}[Feature Space Outlier]
\label{def:FSO}
let $X$ be a data set with features $F$,  $x \in X$ a record and $f \subset F$ a subset of features.\\
$x_f$ is a Feature Space Outlier iff:\\
$$P(x_f | X, f) = \mathbf{low} \\$$
%$$ \left ( \sum_{s \in \mathit{kNN}(x)} dist(s_f, x_f) \right ) > t$$
\end{definition}
That is, when the probability of $x$ in feature space $f$ is low, given the complete dataset and this feature space, we call it a feature space outlier.
However, these featuure space outliers can be ``hidden'' when there are other clusters present in the feature subspace close to the outlying value, in that case the above definition would not hold since the probability given the complete dataset might be normal. We therefor introduce the notion of Local Feature Space Outliers (Definition \ref{def:LFSO}).

\begin{definition}[Local Feature Space Outlier]
\label{def:LFSO}
let $X$ be a data set with clusters $C$, one cluster $c \in C$ and features $F$,  $x \in X$ a record and $f \subset F$ a subset of features.\\
$x_f$ is a Local Feature Space Outlier iff:\\
$$P(x_f | C(x)=c, f) = \mathbf{low}$$
%$$ \left ( \sum_{s \in \mathit{kNN}(x)} dist(s_f, x_f) \right ) > t$$
\end{definition}
In other words, a records' feature space outlier score is depending on the consistency with records that are globally in the same cluster (globally similar).
Note that $C$ does not need to be known, and this can also be one big cluster, in which the definitions above would be the same.

